"Gene": A personal tribute to the Life and Science of Eugene Newman Parker

This review provides a brief account of the life of Eugene Parker (1927-2022) and discusses his contributions to plasma astrophysics. Growing up in Michigan, he went to graduate school at Caltech and then worked at the University of Utah before shifting to the University of Chicago, where he spent the rest of his illustrious career. Parker's most important scientific works are discussed in the context of the historical development of plasma astrophysics. In the study of the Sun, he made enormous contributions both to the MHD of the solar convection zone (including the formulation of turbulent dynamo theory) and to the understanding of the outer solar atmosphere (including the theory of coronal heating and the prediction of the solar wind). Parker's non-solar contributions include the Parker instability in the interstellar gas and the Parker limit of magnetic monopoles. We also try to convey an idea of Parker's highly individualistic personality and his very unique way of doing science.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


